HDMapNet: An Online HD Map Construction and Evaluation Framework

Constructing HD semantic maps is a central component of autonomous driving. However, traditional pipelines require a vast amount of human efforts and resources in annotating and maintaining the semantics in the map, which limits its scalability. In this paper, we introduce the problem of HD semantic map learning, which dynamically constructs the local semantics based on onboard sensor observations. Meanwhile, we introduce a semantic map learning method, dubbed HDMapNet. HDMapNet encodes image features from surrounding cameras and/or point clouds from LiDAR, and predicts vectorized map elements in the bird's-eye view. We benchmark HDMapNet on nuScenes dataset and show that in all settings, it performs better than baseline methods. Of note, our camera-LiDAR fusion-based HDMapNet outperforms existing methods by more than 50% in all metrics. In addition, we develop semantic-level and instance-level metrics to evaluate the map learning performance. Finally, we showcase our method is capable of predicting a locally consistent map. By introducing the method and metrics, we invite the community to study this novel map learning problem.

==> section/algorithm/post_process.tex <==
\begin{algorithm}[h]
\label{alg:post_proces}
\SetAlgoLined
\KwData{segmentation $S$, cluster embedding $C$, direction $D$}
\KwResult{Vectorlized HD Map}
 lines\_cloud = DBSCAN($S$, $C$)\;
 vectorlized\_lines = []\;
 \ForEach{line\_cloud in lines\_cloud} {
 sparse\_line = Directional\_NMS(line\_cloud)\;
 vector\_line = Connect\_Line(sparse\_line, D)\;
 vectorlized\_lines.append(vector\_line)\;
 }
 \Return vectorlized\_lines
 \caption{Vectorization(S, C, D)}
\end{algorithm}



\begin{algorithm}[h]
\SetAlgoLined
\KwData{line point cloud $L$ with confidence}
\KwResult{sparse line point cloud $L'$}
mp\_vertical = MaxPool2d(1, 5)\;
mp\_horizontal = MaxPool2d(5, 1)\;
ap\_vertical = AvgPool2d(5, 9)\;
ap\_horizontal = AvgPool2d(9, 5)\;
L'=L\;
\ForEach{p $\in$ L} {
    \uIf{ap\_vertical(p) $>$ ap\_horizontal(p)}{
        \If{mp\_horizontal(p) != p}{
            drop p from L'\;
        }  
    } \Else{
        \If{mp\_vertical(p) != p} {
            drop p from L'\;
        }
    }
}
\Return L'
\caption{Directional\_NMS(L)}
\end{algorithm}


\begin{algorithm}[h]
\SetAlgoLined
\KwData{line point cloud $L$, direction $D$}
\KwResult{vector line $L'$}
 p = random\_sample(L)\;
 line\_1 = Connect\_One\_Direction(p, L, D)\;
 line\_2 = Connect\_One\_Direction(p, L, D)\;
 vector\_line = concat(line\_1, reverse(line\_2))\;
 \Return vector\_line
 \caption{Connect\_Line(L, D)}
\end{algorithm}


\begin{algorithm}[h]
\SetAlgoLined
\KwData{start point p, line point cloud $L$, direction $D$}
\KwResult{one direction connected vector line $L'$}
 \While{$L$ is not empty} {
    \uIf{Direction pd of p is not taken}{
        pick pd and mark it as taken\;
    } \Else {
        \Break\;
    }

    p\_target = p + pd * step\;
    remove p' in L where dist(p, p') $<$ step-1\;
    p\_next = min(dist(p', p\_target)) where p' in L\;
    \If {dist(p, p\_next) $>$ threshold}{
        \Break
    }
    vector\_line.append(p\_next)\;
    mark the connected direction of p\_next as taken\;
    p = p\_next\;
 }
 \Return vector\_line
 \caption{Connect\_One\_Direction(p, L, D)}
\end{algorithm}


==> section/tables/angle.tex <==
\begin{table}[t]	
\centering
\addtolength{\tabcolsep}{2.5pt}
\begin{tabular}{c|ccccc}
\Xhline{2\arrayrulewidth}
\textbf{\#Angle Class} & 10 & 36 & 90 & 180 & 360 \\ \hline
\textbf{Difference}  & 14.5 & 14.23 & 15.10 & 15.89 & 15.78 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\caption{}
\label{tab:angle_diff}
\end{table}

==> section/tables/sensor_fusion.tex <==
\begin{table*}[tb]	
\centering
\addtolength{\tabcolsep}{0.8pt}
\caption{The results of sensor fusion}
\label{tab:sensor_fusion}
\footnotesize
\scalebox{0.9}{
\begin{tabular}{c c ccc c ccc c ccc}
\Xhline{2\arrayrulewidth}
\multirow{2.5}{*}{\textbf{Method}} & \phantom{a} & \multicolumn{3}{c}{\textbf{{\scriptsize Divider}}} & \phantom{a} & \multicolumn{3}{c}{\textbf{{\scriptsize Ped Crossing}}} & \phantom{a} & \multicolumn{3}{c}{\textbf{{\scriptsize Boundary}}} \\
\cmidrule{3-5} \cmidrule{7-9} \cmidrule{11-13}
&& \textbf{IoU} & \textbf{CD} & \textbf{mAP} && \textbf{IoU} & \textbf{CD} & \textbf{mAP} && \textbf{IoU} & \textbf{CD} & \textbf{mAP}  \\
\hline 
% Softmax && 45.98 $\pm$ 0.79 & 75.25 $\pm$ 0.61 && 58.32 $\pm$ 0.87 & 80.21 $\pm$ 0.59 && 46.87 $\pm$ 0.78 & 67.68 $\pm$ 0.71 \\
% Neg-Softmax && 56.95 $\pm$ 0.82 & 78.87 $\pm$ 0.57 && 59.54 $\pm$ 0.88 & 80.60 $\pm$ 0.57 && 47.74 $\pm$ 0.73 & 68.58 $\pm$ 0.70 \\
% \hline 
% Cosine && 59.49 $\pm$ 0.90 & 79.58 $\pm$ 0.59 &&66.39 $\pm$ 0.93 & 82.17 $\pm$ 0.58 && 42.96 $\pm$ 0.76 & 61.99 $\pm$ 0.75 \\
% Neg-Cosine && 63.68 $\pm$ 0.86 & 82.02 $\pm$ 0.57 && 69.17 $\pm$ 0.85 & 85.60 $\pm$ 0.56 && 44.51 $\pm$ 0.85 & 64.04 $\pm$ 0.75 \\
Camera && 0.406 & 1.740 & 0 && 0.187 & 2.852 & 0 && 0.395 & 1.430 & 0 \\
Lidar && 0.267 & 2.436 & 0.073 && 0.173 & 3.380 & 0.055 && 0.446 & 1.136 & 0.219   \\
Camera \& Lidar && 0.461 & 1.518 & 0.313 && 0.314 & 2.250 & 0.126 && 0.560 & 0.904 & 0.479   \\
\Xhline{2\arrayrulewidth}
\end{tabular}}
\normalsize
\vspace{-10pt}
\end{table*}

==> section/tables/temporal_fusion.tex <==
\begin{table}[t]	
\centering
\addtolength{\tabcolsep}{2.5pt}
\caption{\changed{Temporal fusion on HDMapNet(Surr). The \# of frames means how many frames of samples are fused. 1 means temporal fusion is not used.}}
\begin{tabular}{c|ccc}
\Xhline{2\arrayrulewidth}
\textbf{\# of frames} & 1 & 2 & 4 \\ \hline
\textbf{IoU}  & 32.9 & 35.8 & 36.4 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\label{tab:temporal_fusion}
\vspace{-1em}
\end{table}

==> section/tables/weather.tex <==
\begin{table}[t]	
\centering
\addtolength{\tabcolsep}{2.5pt}
\caption{\changed{The semantic segmentation performance of HDMapNet(Fusion) under different weather condition.}}
\begin{tabular}{c|ccc}
\Xhline{2\arrayrulewidth}
\textbf{Weather} & Night & Rainy & Normal \\ \hline
\textbf{IoU}  & 39.3 & 38.7 & 44.9 \\
\Xhline{2\arrayrulewidth}
\end{tabular}
\label{tab:temporal_fusion}
\vspace{-1em}
\end{table}
